Speaker-independent Speech Separation with Deep Attractor Network

Despite the recent success of deep learning for many speech processing tasks, single-microphone, speaker-independent speech separation remains challenging for two main reasons. The first reason is the arbitrary order of the target and masker speakers in the mixture permutation problem, and the second is the unknown number of speakers in the mixture output dimension problem. We propose a novel deep learning framework for speech separation that addresses both of these issues. We use a neural network to project the time-frequency representation of the mixture signal into a high-dimensional embedding space. A reference point attractor is created in the embedding space to represent each speaker which is defined as the centroid of the speaker in the embedding space. The time-frequency embeddings of each speaker are then forced to cluster around the corresponding attractor point which is used to determine the time-frequency assignment of the speaker. We propose three methods for finding the attractors for each source in the embedding space and compare their advantages and limitations. The objective function for the network is standard signal reconstruction error which enables end-to-end operation during both training and test phases. We evaluated our system using the Wall Street Journal dataset WSJ0 on two and three speaker mixtures and report comparable or better performance than other state-of-the-art deep learning methods for speech separation.

==> Main_singlecol.tex <==
\begin{figure}[!t]
    \centering
    \includegraphics[width=\columnwidth]{pic/danet-flowchart.jpg}
    \caption{The architecture of DANet. The mixture audio signal is projected into a high-dimensional embedding space. The embeddings of time-frequency bins of each speaker are pulled toward reference points called the attractors. During the training phase, the attractors are formed using true or estimated (in anchored DANet) speaker assignments. During the test phase, the attractors are formed in three alternative ways using: unsupervised clustering, fixed points, and anchor points.}
    \label{fig:sys}
\end{figure}

\begin{figure*}[!t]
    \centering
    \includegraphics[width=17cm]{pic/Specgrams.png}
     \vspace{-0.4cm}
    \caption{a) An example of the mixture spectrogram and the recovered speakers. b) Location of T-F bins in embedding space. Each dot visualizes the first three principle components of the embedding of one T-F bin, where colors distinguish the relative power of speakers in that bin. Attractor points are marked with an X.}
    \label{fig:spec}
\end{figure*}

In this section, we introduce the deep attractor network (DANet) \cite{chen2017deep} and compare it to DPCL \cite{hershey2016dpcl} and PIT \cite{kolbaek2017multitalker}. We then discuss three methods for estimating the parameters of the network during test phase and discuss their pros and cons. We further address the limitation of DANet \cite{chen2017deep} by presenting a new framework called ADANet. Figure~\ref{fig:sys} shows the flowchart of the overall system. Note that in this section we use the same notations as in Section~\ref{sec:review}.


\subsection{Model definition}

Following the main concept of embedding learning with neural network, DANet generates a $K$-dimensional embedding vector for each of the T-F bins in the mixture magnitude spectrogram
\begin{align}
 \vec{V} &= f(\vec{x})
 \label{eqn:emb}
\end{align}
where $\vec{V}\in \mathbb{R}^{K\times FT}$ is the embedding matrix containing all the $K$-dimensional embeddings for the T-F bins and $f$ is the mapping function implemented by the neural network. Instead of using affinity matrices to measure the similarity between embeddings \cite{hershey2016dpcl}, DANet uses reference points (\textit{attractors}) in the embedding space to calculate similarity as well as for mask estimation.

An \textit{attractor} $\vec{a}_i \in \mathbb{R}^{1\times K}$ is a vector in the embedding space that represents a specific speaker, such that all the T-F bins belonging to that speaker are pulled toward the corresponding attractor. The attractors are formed during the training phase by calculating the weighted average of embeddings that belong to each speaker:
%\vspace{-0.15cm}
\begin{align}
 \vec{a}_{i}&=\frac{\vec{y}_{i}\vec{V}^{\top} }{\sum_{f,t} \vec{y}_{i}},\quad i = 1, 2, \dotsc, C
 \label{eqn:att}
\end{align}
where $\vec{y}_i \in \mathbb{R} ^{1\times FT}$ denotes the speaker assignment for each T-F bin, which can be either the IBM or IRM in this case (Eqn.~\ref{eqn:allmasks}). Since the attractors represent the centroid of each speaker in the embedding space, averaging over the embeddings that correspond to the most salient T-F bins (i.e. the T-F bins with highest power) may lead to a more robust estimation of the attractors. We therefore apply a threshold to the mixture power spectrogram and create a binary threshold vector $\vec{w} \in R^{1\times FT}$ that filters out the T-F bins with low power. Given a parameter $\rho$, the threshold vector $\vec{w}$ is defined as 
\begin{align}
\vec{w}_{ft} &= 
\begin{cases}
1, \quad \text{if}\quad \vec{x}_{ft} > \rho\\
0, \quad \text{else}
\end{cases}
 \label{eqn:threshold}
\end{align}
%One way to choose $\rho$ is to ensure that a specified percentage of the T-F points are kept after thresholding for each utterance. For example, $90\%$ means a threshold $\rho$ that keeps the top $90\%$ of T-F bins in $X$. 
The attractors are then estimated as follows:
%\vspace{-0.15cm}
\begin{align}
\vec{a}_i&=\frac{(\vec{y}_{i} \odot \vec{w})\vec{V}^\top }{\sum_{f,t} (\vec{y}_{i} \odot \vec{w})},\quad i = 1, 2, \dotsc, C
 \label{eqn:att_weight}
\end{align}

After the generation of the attractors, DANet calculates the similarity between the embedding of each T-F bin and each attractor:
%\vspace{-0.15cm}
\begin{align}
\vec{d}_{i} &= \vec{a}_{i} \vec{V},\quad i = 1, 2, \dotsc, C
\label{eqn:distance}
\end{align}
where $\vec{d}_i\in \mathbb{R}^{1\times FT}$ denotes the distance of each T-F bin in the embedding space from the attractor $i$. This distance $\vec{d}_i$ is small for the embeddings that are close to an attractor, and is large for points that are far away. The mask for each speaker $\hat{\vec{m}}_i \in \mathbb{R}^{1\times FT}, i = 1, \dotsc, C$ is then estimated by normalizing the similarity distance using a nonlinear function to constrain the mask to the range $[0, 1]$
%\vspace{-0.15cm}
\begin{align}
\hat{\vec{m}}_{i}&=\mathcal{H}(\vec{d}_{i}),\quad i = 1, 2, \dotsc, C
\label{eqn:mask}
\end{align}
where $\mathcal{H}$ is a nonlinear function which can be either the Softmax or Sigmoid function that is applied to each element of $\vec{d}_i$:
\begin{align}
\begin{cases}
Softmax(\vec{d}_{i,ft}) = \frac{e^{\vec{d}_{i,ft}}}{\sum_{i=1}^C e^{\vec{d}_{i,ft}}}\\\\
Sigmoid(\vec{d}_{i,ft}) = \frac{1}{\sum_{i=1}^C (1+e^{-\vec{d}_{i,ft}})}
\end{cases}
\label{eqn:activation}
\end{align}

The neural network is then trained by minimizing a standard $L^2$ reconstruction error as the objective function
%\vspace{-0.15cm}
\begin{align}
{l}&=\frac{1}{C}\sum_{i}\left \| \vec{x} \odot (\vec{m}_{i} - \hat{\vec{m}}_{i})\right \|^2_2
\label{eqn:err}
\end{align}
where $\vec{m}_i$ and $\hat{\vec{m}}_i$ $\in \mathbb{R}^{1\times FT}$ are the ideal and estimated target masks for the speakers. Since the masks are a function of both attractors and embeddings, optimizing the reconstruction error (Eqn.~\ref{eqn:err}) forces the network to pull the embeddings that belong to the same speaker together and place the attractors far from each other. The initial embeddings and attractors are randomly distributed in the embedding space, and as the training continues, the attractors gradually become separated and pull the embeddings to a proper space that can separate different speakers. 

The permutation of the speakers in the outputs is determined by the permutation of the attractors in the embedding space. This is further determined by the permutation of the given speaker assignment vectors $\vec{y}_i$. Hence, once the permutation of the target masks $\vec{m}_i$ matches the permutation of speaker assignment function $\vec{y}_i$, we no longer have the permutation problem in DANet. On the other hand, since the number of the speakers is determined by the number of attractors which is a function of $\vec{y}_i$, the output dimension problem is solved in DANet framework, since the number of attractors can change dynamically without changing the network structure. 


\subsection{Relation to DPCL and PIT}

Since DANet shares the same network structure as DPCL \cite{hershey2016dpcl}, it is important to illustrate the difference between DANet and DPCL. In contrast to DPCL, DANet directly optimizes the reconstruction error with a computationally simpler objective function rather than the calculation of affinity matrices in DPCL. Moreover, the direct mask estimation allows it to use flexible similarity measurements and target masks, including phase-aware  \cite{gaich2015phase} and phase-sensitive mask \cite{erdogan2015phase}.

On the other hand, when the attractors are considered as the trained weights of the network instead of dynamically formed by the embeddings (Eqn. ~\ref{eqn:att} \&~\ref{eqn:att_weight}), DANet reduces to a classification network \cite{zhuo2015se,xu2013se} and equation~\ref{eqn:distance} is equivalent to a linear fully-connected layer. In this case, permutation invariant training becomes necessary since the masks are no longer linked to a speaker. However, the dynamic formation of the attractors in DANet allows utterance-level flexibility in the generation of the embeddings. Moreover, DANet does not assume a fixed number of outputs, since the number of attractors is decided by the size of the speaker assignment function $Y$ during training. %In addition, DANet's formation of attractors allows for incorporating speaker dependent knowledge such as the speaker identity, leading to the possibility of constructing speaker-specific attractors. 

==> Reviewer.tex <==
Although all reviewers agree that the proposed approach is interesting, they have some major concerns regarding (i) the clarity of presentation, (ii) the generalization capability of the proposed approach, (iii) the used performance measures, (iv) missing references and comparison to earlier work. As reviewer 2 puts it quite bluntly (but correctly in my opinion), the amount of revision required to bring this manuscript to the standards of TASLP will be substantial. Please especially take care of the following issues in the revised manuscript (note that a point-by-point reply is still required for all reviewer comments):

1) Novelty: please clearly highlight the novelty of this manuscript with respect to your ICASSP 2017 paper (reviewer 1 and 2)

2) Presentation: all reviewers agree that the clarity of presentation needs to be drastically improved and a lot of important details need to be mentioned/explained. E.g., all mathematical symbols need to be defined, mathematical mistakes need to be corrected, all of the compared methods should be briefly described or cited, the evaluation conditions (STFT size, SNR, ...) should be clearly mentioned.

3) Generalization capability of the proposed approach, especially regarding the number of sources in training and evaluation and the optimization of the hyperparameters (reviewer 3).

4) Evaluation/performance measures (reviewers 1 and 2): please use standard performance measures (e.g., from the BSS Eval Toolbox) instead of defining your own measures. In addition, please also report PESQ results in addition to SDR. The suggestion of reviewer 2 to also present IRM results is optional in my opinion.

5) Missing references to earlier work. The authors need to place their work in context, in addition to deep clustering and PIT.
********

Your revised manuscript must be submitted back to ScholarOne Manuscripts https://mc.manuscriptcentral.com/tasl-ieee no later than 6 weeks from the date of this letter together with a required point-by-point reply that explains how you addressed the reviewers' comments. If we do not receive your revised manuscript within 6 weeks from the date of this letter, your manuscript will be considered withdrawn.

After you finish revising your manuscript, please log into your Author Center at https://mc.manuscriptcentral.com/tasl-ieee to upload the new file(s) to your submission. You will find your manuscript title listed under "Manuscripts with Decisions."  Under "Actions," click on "Create a Revision.”

When submitting your revised manuscript, please make sure to also upload your required “response-to-reviewers” file. You can upload this file in the section marked “Respond to the Decision Letter” or to the “File Upload” section. It must be uploaded as a separate file from your manuscript file. Please do NOT upload it to the “cover letter” field as the AE/reviewers do not have access to that section.

Please remember that the Associate Editor should only decide RQ (major revision) once during the peer review process of any paper. Subsequent decisions after one RQ should be AQ, A, or R only.

If you have any questions regarding the reviews, please contact me. Any other inquiries should be directed to Kathy Jackson.

NOTE – Open Access:
The publication is a hybrid journal, allowing either Traditional manuscript submission or Open Access (author-pays OA) manuscript submission. Upon submission of your final files, if you choose to have your manuscript be an Open Access article, you commit to pay the discounted OA fee if your manuscript is accepted for publication in order to enable unrestricted public access. As of 01 January 2017, the OA fee is $1,950. Any other application charges (such as charge for the use of color in the print format) will be billed separately once the manuscript formatting is complete but prior to the publication. If you would like your manuscript to be a Traditional submission, your article will be available to qualified subscribers and purchasers via IEEE Xplore. No OA payment is required for Traditional submission.

NOTE – Overlength manuscripts:
The final submitted version of your manuscript may not exceed 16 pages in the double-column, single-spaced format including figures, photos, and bios. If your paper is accepted, it will not be sent to production if it exceeds this limit. Additionally, any manuscript that exceeds 10 pages in double-column format will be charged mandatory overlength fees. The rate is $220/page starting on page 11 of a published manuscript.

================================================


Best regards,

Prof. Simon Doclo
Associate Editor
IEEE Transactions on Audio, Speech and Language Processing
simon.doclo@uni-oldenburg.de, simon.doclo@ieee.org

Kathy Jackson
Coordinator Society Publications
IEEE Signal Processing Society
k.jackson@ieee.org

Reviewer Comments:

Reviewer: 1

Recommendation: RQ - Review Again After Major Changes

Comments:
Please find my comments in the attached PDF document.

Additional Questions:
1. Is the topic appropriate for publication in these transactions?: Excellent Match

1. Is the paper technically sound?: Yes

2. How would you rate the technical novelty of the paper?: Somewhat Novel

3. Is the contribution significant?: Incremental

4. Is the coverage of the topic sufficiently comprehensive and balanced?: Important Information is missing or superficially treated

5. Rate the Bibliography: Unsatisfactory

1. How would you rate the overall organization of the paper?: Could be improved

2. Are the title and abstract satisfactory?: Yes

3. Is the length of the paper appropriate? If not, recommend what should be added or eliminated.: Yes

4. Are symbols, terms, and concepts adequately defined?: Not always

5. How do you rate the English usage?: Needs improvement


Reviewer: 2

Recommendation: RQ - Review Again After Major Changes

Comments:
This paper presents a neural network based method to separate multiple speakers. The main idea is the so-called attractor network for speaker-independent separation. While the idea has some merit and obtained results seem reasonable, the paper contains problematic assertions and is not properly placed in the context of considerable recent work in deep learning based speech separation. Furthermore, many important details are missing. In addition, the work is narrowly focused and the presentation leaves much to be desired. I have got an impression that the authors take a casual approach towards paper writing. Although my recommendation is Major Revision, I am torn between it and rejection, as I believe that the amount of revision required to bring this submission to the standards of this Transactions is substantial. If the decision is revision, the authors should be allowed an extension beyond the standard 6 weeks for the revision. Here are my detailed comments:

-       The authors must quote their own ICASSP’17 paper, and clarify the novelty of this work relative to their ICASSP paper. Not mentioning their ICASSP paper is not excusable.

-       The use of the term “attractor” is problematic. To my knowledge, an attractor is a mathematical concept that refers to a stable fixed point, where initial points of a dynamical system converge to through evolution. This is also a popular term in neural networks, but it refers to stored patterns in the Hopfield associative memory. In this study, the term seems to refer to just cluster centers and there is no dynamical pulling or evolution. As such, the use of the term appears to be a misnomer, the reference [18] notwithstanding. I suggest that the authors think of a more accurate name to avoid confusion.

-       They should quote the recently published journal version of the PIT technique (Kolbak et al.’17, in this Transactions, i.e. T-ASLP). Their authors also have an earlier version in ICASSP’17. This manuscript only quotes a 2016 preprint. The comparisons with PIT in this paper should be updated accordingly.

-       As reported in Kolbak et al.’17, the PIT method can be applied to separation of combined 2 and 3 speakers. Their SDR results appear to be a little better than those shown in Table V. The authors should expand Table V to include a comparison with Kolbak et al.

-       In terms of evaluation, the paper should report PESQ results in addition to SDR. The problem with SDR and SNR is that their relevance to the end use of speech separation, i.e. better speech intelligence or quality, is unclear. PESQ is a standard quality metric, and is used in Kolbak et al. In addition, IRM results should be reported so that the reader can easily see the gap from the ceiling performance.

-       The authors make no attempt to explain why speaker-independent separation is a significant problem to study, in the context of earlier work on speaker-dependent and target-dependent talker separation work. Relevant work by Huang et al.: “Joint optimization of masks and deep recurrent neural networks for monaural source separation,” T-ASLP’15, by Zhang and Wang: “A deep ensemble learning method for monaural speech separation,” T-ASLP’16, and by Du et al.: “A regression approach to single-channel speech separation via high-resolution deep neural networks,” T-ASLP’16 should be discussed. The authors’ attempt at an explanation in the fifth paragraph of Sect. I is confusing and not to the point. This has to be rectified.

-       Likewise, prior to DNN, multi-talker speaker-independent separation has been approached using spectral clustering (Bach and Jordan: “Learning spectral clustering, with application to speech separation,” JMLR’06), NMF (Smaragdis: “Convolutive speech bases and their application to supervised speech separation,” T-ASLP’07), and CASA (see Hu and Wang: “An unsupervised approach to cochannel speech separation,” T-ASLP’13). The authors need to place their work in this context, in addition to deep clustering and PIT.

-       Many details are missing. A good journal article should be self-contained and include enough detail to enable replication by an interested reader. A lot of things are left unexplained in this manuscript, including:

o       The softmax function should be defined

o       Each of the compared methods should be described, including DPCL++ and PIT-T-BLSTM-ST (what is ‘ST’?)

o       What are DANet 4 and DANet 5?

o       Where is Fig. 4 explained?

o       In your evaluation with 2 and 3 speakers, what are input SNRs? Is each utterance equally loud in a multitalker mixture?

-       A number of claims made in this MS are incorrect or problematic:

o       Sect. I, third paragraph, the citations to statistical methods are problematic. For example, [5] is a multichannel method. Treating [6] as a statistical method and in the next paragraph as a deep learning method is misleading. Also, a paper using NMF for speech separation should be quoted instead of [8], which is on NMF itself.

o       Next paragraph, the statement that auto-encoders are the most commonly used deep learning approach to speech separation is simply false and illustrates the weak command of relevant literature by the authors. The most commonly used approach is time-frequency masking, i.e. using deep learning to estimate an ideal T-F mask, of which this manuscript is an example. Again, the cited papers are unrepresentative, and should include the first such study (Wang and Wang: "Towards scaling up classification-based speech separation," T-ALSP’13).

o       P. 2, second paragraph, the statement that PIT assumes a fixed number of sources should be qualified in light of Kolbak et al. mentioned above. Note that your method seems to also assume the number of speakers, i.e. parameter C in your formulation.

o       By an end-to-end separation system, people usually refer to time-domain separation, i.e. at the waveform level. My understanding is that your algorithm operates in the STFT domain and needs to take noisy speech phase in order to reconstruct the time domain signal.

-       The following is a list of minor writing issues:

o       Line 9 of abstract: ‘projects’ -> ‘project’
o       Still in abstract: remove one ‘both’ out of its two occurrences in the same sentence
o       Two paragraphs after (1), remove one ‘only’ out of its two occurrences in the same sentence
o       Paragraph after (5): ‘compare’ -> ‘compared’
o       Paragraph after Fig. 3: remove ‘can’ before ‘needs’
o       Last sentence of paragraph 2 of Sect. IV.B: it basically repeats the previous one
o       Last paragraph of p. 5: remove one ‘the’ out of its two occurrences in the same sentence
o       First sentence of Sect. V.C: ‘threshold’ -> ‘thresholds’
o       P. 8, first sentence: check for multiple errors
o       Last sentence of the same paragraph: ‘expect’ -> ‘except’
o       Ref. 1: ‘Sachieving’?


Additional Questions:
1. Is the topic appropriate for publication in these transactions?:

1. Is the paper technically sound?:

2. How would you rate the technical novelty of the paper?:

3. Is the contribution significant?:

4. Is the coverage of the topic sufficiently comprehensive and balanced?:

5. Rate the Bibliography:

1. How would you rate the overall organization of the paper?:

2. Are the title and abstract satisfactory?:

3. Is the length of the paper appropriate? If not, recommend what should be added or eliminated.:

4. Are symbols, terms, and concepts adequately defined?:

5. How do you rate the English usage?:


Reviewer: 3

Recommendation: RQ - Review Again After Major Changes

Comments:
This method presents an end-to-end training method to improve the performance of deep clustering.

I recommend a major revision of the paper concerning the following points:

- The presentation needs to be improved. Mainly, it is not clear how the algorithm generalizes to a number of sources that has not been seen in training. It would be very helpful to have a list of variables which are parameters of the network ("weights"), and which are re-computed for each utterance ("activations").

- Along these lines, the performance needs to be compared to deep clustering on a mismatched training/test scenario, e.g., training on mixtures of 2 speakers and testing on mixtures of 3 speakers.

- Many more comments on clarity, mathematical soundness and mode of presentation can be found in the attached PDF.

- In a similar vein, it is not clear how different numbers of sources are handled in training, since this changes the dimension of, e.g., the matrix A. Are the parameters shared between the A matrix used for 2 sources and 3 sources, or are there different matrices for different numbers of sources?

- The optimization of the hyperparameters is only done on the test set. This can over-estimate the performance. For example, the number of anchor points and the usage of dropout needs to be validated on the validation set, before evaluating on the evaluation set.



Additional Questions:
1. Is the topic appropriate for publication in these transactions?: Excellent Match

1. Is the paper technically sound?: Yes

2. How would you rate the technical novelty of the paper?: Novel

3. Is the contribution significant?: Moderately Significant

4. Is the coverage of the topic sufficiently comprehensive and balanced?: Yes

5. Rate the Bibliography: Satisfactory

1. How would you rate the overall organization of the paper?: Could be improved

2. Are the title and abstract satisfactory?: Yes

3. Is the length of the paper appropriate? If not, recommend what should be added or eliminated.: No (Explain):

4. Are symbols, terms, and concepts adequately defined?: Not always

5. How do you rate the English usage?: Needs improvement

==> response_Yi.tex <==
Dear Prof. Simon Doclo,

Thanks for the valuable advices by you and all the reviewers. Please allow me to first address our changes to the major concerns, and then reply point-by-point on each of the comments made by the reviewers.

1) Novelty: We now reframe the model part into two more distinct sections: the original DANet proposed in our ICASSP 2017 paper, and the improved model to fix several issues in DANet, which we refer as anchored DANet (ADANet). Section II includes the details about the problem setting of source separation and the application of embedding learning in this problem, and in Section III we introduce the problems and how to tackle them. We think the difference and improvement of this work comparing with the ICASSP paper is more clear now.

2) Presentation: We rewrite the entire Section II, III and IV to fix the mathematical symbols, equations and the information flow. The details of the experiment settings are also added in Section V.

3) Generalization and hyper-parameters: We make it more clear about the speaker setting in different experiments and datasets. We re-designed the experiment for the mixed speaker scenario, i.e. when mixture has either 2 or 3 speakers, to have a better comparison with previous systems. The hyper-parameter setting and the algorithm used for optimization are also in Section V.

4) Evaluation performance: We add the performance on standard BSS evaluation metrics to compare with PIT, and keep the original evaluation metric (i.e. scale-invariant SNR) to compare with deep clustering. We also added the PESQ scores of different configurations of our network in Table III. One concern we have about PIT is that we are not certain about the definition of 'PESQ improvement' in Kolbak et al.'s PIT paper. They mentioned that ideal ratio mask (IRM) has a 2.11 PESQ ``improvement'', while in our experiments using ITU-T Recs P.862 PESQ, the PESQ ``score'' of ideal wiener-filter is 2.03. So we are wondering if the reported number of IRM and the separated results are PESQ ``score'' or PESQ ``improvement''. Here we report our results by PESQ scores without comparing with their numbers.

5) Missing references: The reason we put more focus on deep clustering and PIT is that they are the most recent works that proposed and tried to tackle the permutation problem and output dimension problem, and our approach is closely related to these two works. To have a better connection and comparison of these two methods with previous approaches, we make changes to the introduction section in order to have a transition from previous works to these two works, and then introduce our approach based on theirs.

Point-by-point reply:

Reviewer 1:

Reviewer 1 said that the detailed comments is in an attachment, but we did not receive that in the email. We will reply to it as soon as we receive the attached file.

Reviewer 2:

 - We added the citation of the ICASSP 2017 paper, and Section III discussed its main disadvantages and introduced the improved version of the model.
 
 - The use of term 'attractor' is mainly inspired from the perceptual magnet effect, where the embeddings of one speaker is gradually 'attracted' to a point in the embedding space as the training procedure continues. The calculation of attractors in our context is indeed the center of a group of embeddings, but through the calculation of the distance between embeddings and the attractors, the attractors explicitly force the embeddings to gather around in order to generate proper masks. From the perspective of the evolution of network training, the initial embeddings and attractors and randomly distributed in the embedding space, and as the training continues, the attractors gradually attract the embeddings to a proper space that can separate different speakers. This is similar to the convergence of a dynamic system, where the fix points are the attractors in our case. 
 
 - We fixed the citations of inproper preprint versions and updated the results in the experiment part accordingly.
 
 - To make a comparison with PIT of the mixed speaker condition (i.e. 2+3 speaker condition), we re-designed and re-trained our network in a similar fashion with PIT. The comparison of the results is in Table V.
 
 - The main drawback of speaker-dependent separation is that it requires the information of speaker to be known during both training and test phase. However, in real-world situations, speaker information are typically unknown. Moreover, human brain can perform speaker-independent separation with easy in most of the scenarios. 
 
 - The citations of other related works have been added to discussion in Section I.
 
 - About the details of the paper:
    o We think the definition and usage of softmax function in deep learning is widely known, so we did not put the definition here. Moreover, in other publications such as Kolbak et al.'s PIT paper, activation functions such as sigmoid, softmax and ReLU were directly mentioned without definition. But for clarification, we add the definition of softmax in Eqn. 13.
    
    o We add descriptions about all the methods we compare with.
    
    o The naming of different network configurations are fixed in the experiment section.
    
    o Fig. 4 is now explained in Section III.C.
    
    o The dataset setting, network configuration are described in detail in Section V.
    
    o It might be somehow misleading to use 'autoencoder-type network' to indicate an approach. We changed it to mention the most commonly used 'network structure' in deep learning studies. Time-frequency masking is the generalized approach toward the separation problem without limiting to deep learning based systems, and our aim in Section I paragraph 3 is to focus on deep learning systems. We were not trying to pose autoencoder at the top of T-F mask estimation, and we also fixed the way we convey it. The citation of the first work is also added.
    
    o The number of speakers was needed in both our approach and PIT during training, and we added one more experiment similar to PIT to confirm that during test time the number of sources is not necessary. The corresponding statements about PIT is also fixed.
    
    o The use of end-to-end here is following the usage of Isik et al., "Single-Channel Multi-Speaker Separation using Deep Clustering", where the input and output of the networks were both magnitude spectrograms. The term 'end-to-end' here is to distinguish it from the previous version, where a post-clustering step is needed to generate the masks.
    
    o The writing issues have been fixed.
    
    
Reviewer 3:

 - We make it more clear in Section V about the detailed configuration of the networks. We only use 2 or 3 speaker mixtures for evaluation to have a fair comparison with previous methods, but we re-designed the experiment about the mixed speaker case, i.e. use a same network to separate either 2 or 3 speaker mixtures.
 
 - Since the training of our system is end-to-end, it's somehow unimportant to evaluate the system in mismatched condition similar to the original deep clustering. With end-to-end optimization and evaluation, the embeddings are optimized to direct generate the masks, while in the none end-to-end deep clustering configuration, the embeddings were only optimized to better fit the affinity matrix and is somehow independent from the masks. The use of affinity as the objective made deep clustering 
 
 - Mathematical symbols and writing issues have been fixed.
